Learning-Augmented Metric Distortion via $(p,q)$-Veto Core

In the metric distortion problem there is a set of candidates $C$ and voters $V$ in the same metric space. The goal is to select a candidate minimizing the social cost: the sum of distances of the selected candidate from all the voters, and the challenge arises from the algorithm receiving only ordinaL input: each voter's ranking of candidate, while the objective function is cardinal, determined by the underlying metric. The distortion of an algorithm is its worst-case approximation factor of the optimal social cost. A key concept here is the (p,q)-veto core, with $p\in \Delta(V)$ and $q\in \Delta(C)$ being normalized weight vectors representing voters' veto power and candidates' support, respectively. The (p,q)-veto core corresponds to a set of winners from a specific class of deterministic algorithms. Notably, the optimal distortion of $3$ is obtained from this class, by selecting veto core candidates using uniform $p$ and $q$ proportional to candidates' plurality scores. Bounding the distortion of other algorithms from this class is an open problem. Our contribution is twofold. First, we establish upper bounds on the distortion of candidates from the (p,q)-veto core for arbitrary weight vectors $p$ and $q$. Second, we revisit the metric distortion problem through the \emph{learning-augmented} framework, which equips the algorithm with a (machine-learned) prediction regarding the optimal candidate. The quality of this prediction is unknown, and the goal is to optimize the algorithm's performance under accurate predictions (consistency), while simultaneously providing worst-case guarantees under arbitrarily inaccurate predictions (robustness). We propose an algorithm that chooses candidates from the (p,q)-veto core, using a prediction-guided q vector and, leveraging our distortion bounds, we prove that this algorithm achieves the optimal robustness-consistency trade-off.

==> sections/40-optimal_algorithm.tex <==
\section{The Boosted Simultaneous Veto ($\SimVeto$) Algorithms}
\label{sec:optimal_algorithm}

In this section we present a family of algorithms termed $\SimVeto$, parametrized by $\delta \in\left[0,1\right)$. 
Our main result shows that for each choice of $\delta \in \left[0,1\right)$, $\SimVeto$ achieves an optimal trade-off point between robustness and consistency:

\begin{theorem}
\label{thm:optimal_algorithm}
    For any $\delta \in \left[0,1\right)$, $\SimVeto$ achieves $\frac{3-\delta}{1+\delta}$-consistency and $\frac{3+\delta}{1-\delta}$-robustness.
\end{theorem}

In what follows, we provide a description of the algorithm $\SimVeto$, followed by several observations. A pseudo code for the algorithm appears as Algorithm~\ref{alg:simultaneous_veto} and an execution example is described in Figure \ref{fig:example}.

\paragraph{$\SimVeto$ algorithm.} The algorithm initializes scores for the candidates --- each candidate other than the prediction starts with score equal to its plurality score.  The predicted candidate's initial score is boosted and equals its plurality score plus some boost $\boost = \frac{2\delta n}{1-\delta}$.
We say that a voter $v$ \textit{up-votes} a candidate $c$ if $\topc(v) = c$.
Note that the sum of initial scores equals $n + \boost = \boosttotal n$.

\begin{figure}[h]
    \centering
    \includegraphics[width = \textwidth]{images/bigpicv2.png}
    \caption{Four figures visualizing the execution of $\SimVeto$ for $\delta=1/3$ on an instance with 5 candidates and $n=3$
    voters. The first figure, at $t=0$, exhibits each voter's up-vote and each candidate's intial score (candidate $\p$ has a boosted score of $0+\frac{2\delta n}{1-\delta} = 3$). 
    The voters then down-vote at rate $\frac{1+\delta}{1-\delta}=2$.
    The other three figures exhibit the down-vote of the voters in each of the three rounds of $\SimVeto$ before all scores reach 0.
    Time points $t_1,t_2,t_3$ mark the end of each round.} 
    \label{fig:example}
\end{figure}
After the initialization stage, from time $t = 0$ until $t = 1$, the voters continuously and simultaneously ``eat'' (decrement) the score of their least-favorite candidate that still has positive score, at a rate of 
$(n+\boost)/n = \boosttotal$.
We say that a voter $v$ \textit{down-votes} some candidate $c$ whenever $v$ decrements $c$'s score.
We say that a candidate is \textit{active} at some time point if her score at that time point is positive.
Each time that the score of some candidate reaches 0, all voters that down-voted it up to that point immediately switch to down-voting their next least-favorite active candidate.

Observe that the first (and only) time point at which all candidates reach score 0 is the end of the algorithm ($t = 1$).
If the predicted candidate is one of those that reached score 0 only at the end, then it is output.  Otherwise, the algorithm chooses some arbitrary candidate whose score reached 0 only at the end. In particular we have
\begin{observation}\label{obs:winnerpositivescore} 
\label{obs:winner_active}
    For any $\delta \in [0,1)$,
    the candidate output by a given execution of $\SimVeto$ is active
    at any time point $t < 1$.
\end{observation}


\paragraph{A discrete implementation of $\SimVeto$.}
We implement the continuous process described above 
in a sequence of up to $m$ rounds
which are divided by time points at which the score of some candidate reaches 0 ---
at least one candidate is eliminated at the end of each round.
Round $i$ starts at time $t_{i-1}$ and ends at time $t_i$, where $t_0 = 0$, and $t_k = 1$ where $k$ is the total number of rounds.
Given $t_{i-1}$, we determine $t_i$ as follows:

Let $\score(c)$ be the current score of candidate $c$ at time $t_{i-1}$, and let $n_c$ be the number of voters whose least favorite active candidate at time $t_{i-1}$ is $c$ --- these are the voters who are currently 
down-voting $c$.
Let $\Tilde{c}$ be a candidate minimizing the ratio $\Delta = \score(c)/\left(n_c \cdot \boosttotal\right)$.  This is the time interval 
until the next time point at which
some candidate's score reaches 0.  $t_i = t_{i-1} + \Delta$ is the new time point, and a new round begins after appropriately updating the scores of all candidates.
All voters who in the previous round were down-voting a candidate whose score reached zero at exactly this point switch to down-voting their next least favorite active candidate in the new round. We emphasize that more than one candidate may become inactive at the end of a round, in which case the number of rounds $k$ is strictly less than $m$.

\begin{algorithm}[h]
\DontPrintSemicolon
\KwIn{Preference profile $\sigma$, predicted optimal candidate $\p\in \C$}
\KwOut{a candidate $c \in \C$}
\;
\tcc{All candidates start with score equal to their plurality, except for $\p$ who gets boosted.}
\Initialize{
$\forall c \in \C \setminus \{\p\}$, $\mathsf{score}(c) \gets \plu(c)$, \;
$\score(\p) \gets \plu(\p) + \boost$, where $\boost = \frac{2\delta n}{1 - \delta}$. \;
$i \gets 1$ \;
$t_0 \gets 0$ \;
}
\tcc{Voters decrement the score of their least-favorite candidate that still has positive score, continuously and \mfe{simultaneously,}
at rate $\boosttotal$. Following is a discrete implementation:}
\While{$\exists c \in \C \text{ s.t. } \score(c) > 0$}{
    $A \gets \{c \in \C \mid \score(c) > 0\}$ \tcp*{Set of current active candidates}
    $\forall c \in \C: n_c \gets \left|\{v \in \V \mid \botc_A(v) = c\}\right|$ \tcp*{Number of current "down-voters" for each candidate $c$}%\;
    $\Delta \gets \min_{c \in A} \frac{\score(c)}{n_c \cdot \left(\boosttotal\right)}$ \tcp*{Time interval until some candidate's score reaches 0}%\;  
    $t_i \gets t_{i-1} + \Delta$ \tcp*{Time point when this happened}
    $\forall c \in \C: \score(c) \gets \score(c) - \Delta\cdot n_c \cdot \left(\boosttotal\right)$ \tcp*{Appropriate score updates}%\;
    $i \gets i+1$
}
\tcc{All candidates now have score 0.\ $A$ contains only candidates whose score reached 0 at $t=1$}
\If{$\p \in A$}{
    \textbf{return }$\p$
}
\Else {
    \textbf{return} an arbitrary $c \in A$
}
\caption{$\SimVeto$}
\label{alg:simultaneous_veto}
\end{algorithm}

\begin{definition}
Given an execution of $\SimVeto$, 
we use $f(v,c)\in [0,1]$ to denote the fraction of time that each voter $v\in \V$ spends down-voting each candidate $c\in \C$ throughout the execution. Since every voter spends all the $[0,1]$ time interval down-voting at a rate of $\frac{1+\delta}{1-\delta}$
and since every candidate's score eventually reaches $0$, we have
\begin{align}
\sum_{c\in \C}f(v,c)&=1 &\text{ for every voter  $v$,}\label{Eq:total_time}\\
\sum_{v\in\V} f(v,c) &= \frac{1-\delta}{1+\delta}\cdot \plu(c)   &\text{for every candidate $c\neq\p$, and}\label{Eq:total_downvote1}\\
\sum_{v\in\V} f(v,\p) &= \frac{1-\delta}{1+\delta}\cdot \left(\plu(\p)+\y\right)   &\text{for the predicted candidate $c=\p$.}\label{Eq:total_downvote2}
\end{align}
\end{definition}


\begin{lemma}\label{lem:activecandidate}
For any $\delta \in [0,1)$,
let $a$ be the candidate output by a given execution of $\SimVeto$.  Then, for any voter $v$ and any candidate $c$ satisfying $f(v,c) >0$, we have $d(v,c) \geq d(v,a)$.
\end{lemma}
\begin{proof}
First by Observation~\ref{obs:winnerpositivescore} we know that 
$a$ is active throughout the algorithm, {\sl i.e.}
$a \in A$ 
in all rounds of the algorithm.
Since $f(v,c) >0$, we have $c 
 = \botc_A(v)$
 in at least one of the rounds.
 By definition of $\botc_A$, we have $d(v, c) \geq d(v,a)$.
\end{proof}

The remainder of this section is organized as follows.
In Section \ref{sec:consistency} we establish our consistency bound. 
The more challenging part is the robustness bound, which is established in the following subsections. 
In Section \ref{sec:robustness_prediction} we establish our robustness bound for instances where the predicted candidate is returned by the algorithm. 
This bound is then extended in Section~\ref{sec:robustness_not_prediction} 
to all instances, by reducing any instance to one where the predicted candidate is returned.

==> sections/43-consistency.tex <==
\subsection{Consistency Bound}
\label{sec:consistency}
\begin{proposition}
\label{prop:consistency}
    For any $\delta \in [0,1)$, 
    let $a$ be the candidate output by a given execution of $\SimVeto$ that is provided with the correct prediction $\p = \o$.
    Then we have
    $$\SC(a) \leq \frac{3-\delta}{1+\delta}\cdot \SC(\o).$$
\end{proposition}
\begin{proof}
The social cost of the returned candidate $a$ can be upper bounded as follows:
{\allowdisplaybreaks
\begin{align*}
    \sum_{v} d(v,a) &\leq \sum_v\sum_c f(v,c) \cdot d(v,a) \tag{using \eqref{Eq:total_time}}\\
    & \leq \sum_v \sum_c f(v,c) \cdot d(v,c) \tag{by Lemma~\ref{lem:activecandidate}}\\
    & \leq \sum_v\sum_c f(v,c) \cdot (d(v,\o) + d(\o,c)) \tag{triangle inequality}\\
    & = \SC(\o) + \sum_c \sum_v f(v,c) \cdot d(\o,c)\\
    & = \SC(\o) + \sum_{c\neq \o} \sum_v f(v,c) \cdot d(\o,c) \tag{since $d(\o,\o)=0$}\\
    & = \SC(\o) +\sum_{c\neq \o} \frac{1-\delta}{1+\delta}\cdot \plu(c)\cdot d(\o,c) \tag{using~\eqref{Eq:total_downvote1} and the fact that $\p = \o$}\\
    & =\SC(\o) + \frac{1-\delta}{1+\delta} \sum_{c}\sum_{v: \topc(v) = c}d(\o,c) 
    \\
    & \leq \SC(\o) + \frac{1-\delta}{1+\delta} \sum_{c}\sum_{v: \topc(v) = c}d(\o,v) + d(v,c) \tag{triangle inequality}\\
    & \leq  \SC(\o) + \frac{1-\delta}{1+\delta} \sum_{c}\sum_{v: \topc(v) = c} 2d(\o,v) \tag{since $c= \topc(v) \pref_v \o$}\\
    & \leq \SC(\o) + \frac{2(1-\delta)}{1+\delta}\SC(\o)
    \leq \frac{3-\delta}{1+\delta}\SC(\o). \qedhere
\end{align*}}

\end{proof}

==> sections/46-robustness.tex <==
\subsection{Robustness Bound when the Returned Candidate is the Prediction}\label{sec:robustness_prediction}
\begin{proposition}
\label{prop:robustness_main}
        For any $\delta \in [0,1)$, 
        assume that $\p$ is the candidate output by a given execution of $\SimVeto$,
        {\sl i.e.}, the algorithm returns the prediction.
        Then we have
        $$\SC(\p) \leq \frac{3+\delta}{1-\delta} \cdot \SC(\o).$$
\end{proposition}

To prove Proposition~\ref{prop:robustness_main}, {\sl i.e.}, the upper bound on $\SC(\p)/\SC(\o)$ stated above, the key technical contribution of this section is 
establishing an upper bound on the distance between the optimal candidate, $\o$, and the prediction, $\p$, as a function of the optimal social cost (see Lemma~\ref{lem:keylemma}). To prove this upper bound, we define a graph (the \emph{veto map}) that captures the way in which the down-voting of each voter is distributed across the up-votes of other voters and then use the structure of this graph to appropriately lower bound the distance of (pairs of voters) from the optimal candidate, $\o$ (see Lemma~\ref{lem:1-1matching}).

\begin{figure}[h]
    \centering
    \includegraphics[width = \textwidth]{images/sec42pic.png}
    \caption{Revisiting the instance of Figure~\ref{fig:example}, each of the first three figures exhibits the values of $f(v,c)$ for a distinct voter $v$, and the third figure provides the induced veto map among the voters.}
    \label{fig:vetomap}
\end{figure}

\begin{definition}[The Veto Map]
Let $\delta \in [0,1)$.
Given an execution of $\SimVeto$, the \emph{veto map} associated with this execution is an edge-weighted directed graph $G = (\V, E)$, where each vertex corresponds to a voter in $\V$ and an edge $(v,v')$ between two voters $v,v'\in \V$ exists in $E$ if and only if voter $v$ down-voted the top candidate of $v'$ at some point during the execution, {\sl i.e.}, if and only if $f(v,\topc(v'))>0$. The weight of each edge $(v,v')\in E$ is 
\begin{equation}\label{eq:edge_weight}
w(v,v')\vcentcolon=\frac{f(v,\topc(v'))\cdot\frac{1+\delta}{1-\delta}}{\plu(\topc(v'))}.
\end{equation}
\end{definition}

Note that for each edge $(v,v')\in E$, the numerator of~\eqref{eq:edge_weight} is equal to the amount by which voter $v$ decreased the score of candidate $\topc(v')$ throughout the execution of $\SimVeto$ ({\sl i.e.}, the amount of time, $f(v,\topc(v'))$, that $v$ spent down-voting that candidate, multiplied by the rate, $(1+\delta)/(1-\delta)$). The denominator of~\eqref{eq:edge_weight} is the plurality of this candidate, {\sl i.e.}, the number of voters who up-voted her. Therefore, for each voter $v$ and each candidate $c$, the veto map essentially ``distributes'' the  amount by which $v$ reduced the score of $c$ equally among the weights of the edges from $v$ to each voter $v'$ such that $c=\topc(v')$, {\sl i.e.}, each voter that up-voted $c$. Figure~\ref{fig:vetomap} provides the veto map for the example introduced in Figure~\ref{fig:example}.

We now make the crucial observation that for every edge $(v,v')\in E$ ({\sl i.e.}, for every edge of the veto map), we can derive a lower bound on the combined contribution of voters $v$ and $v'$ to the social cost of the optimal candidate, $\o$. Intuitively, if $v$ down-voted the candidate closest to $v'$ (this is the meaning of the assumption that $(v,v') \in E$),
then $v$ must be far enough from that candidate and hence from $v'$ as well.  In turn, if one of $v$ or $v'$ is close to $\o$ then the other voter must be far enough from $\o$.
\begin{lemma}\label{lem:1-1matching}
For any $\delta \in [0,1)$, 
let
$G=(\V,E)$ 
be the veto map
associated with a given execution of $\SimVeto$.  If $(v,v') \in E$, then we have $d(v,\o) + d(v',\o) \geq \frac{d(\o, p)}{2}$.
\end{lemma}
\begin{proof}
Consider any $v$, by the triangle inequality we have 
\begin{align}\label{eq:triangleinequality}
  d(\o,p) \leq d(p,v) + d(v,\o) ~\Rightarrow~ d(p,v) \geq d(\o,p) - d(v,\o).  
\end{align}
By definition of the veto map, the fact that $(v,v') \in E$ implies that voter $v$ down-voted the top candidate of $v'$. Let $c = \topc(v')$. We have
\begin{align}\label{eq:candidatesum}
    d(\o, c) ~\geq~ d(c,v) - d(v,\o) ~\geq~ d(\p,v) -d(v,\o) ~\geq~ d(\o,\p) -2d(v,\o),
\end{align}
where the first inequality holds by the triangle inequality, the second holds since $d(c,v) \geq d(\p,v)$ by Lemma \ref{lem:activecandidate}, and the last inequality is using~\eqref{eq:triangleinequality}. Now consider voter $v'$, we have
\begin{align*}
 d(\o,v') + d(v',c) &\geq d(\o,c) &\text{(by triangle inequality)} ~~~&\Rightarrow \\
 2d(\o,v') &\geq d(\o,c) &\text{(since $c = \topc(v') \pref_{v'} \o$)}  ~~~&\Rightarrow \\
  2d(\o,v') &\geq d(\o,\p) - 2d(v,\o)  &\text{(using \eqref{eq:candidatesum})}~~~&\Rightarrow\\
  d(\o,v)+d(\o,v') &\geq \frac{d(\o,\p)}{2}. \qedhere
\end{align*}
\end{proof}


Using the veto map and Lemma~\ref{lem:1-1matching}, we can now prove the key lemma of this section (Lemma~\ref{lem:keylemma}), which provides a lower bound of $\left(\frac{1-\delta}{2}n\right)\frac{d(\o,p)}{2}$ on the optimal social cost, $\SC(\o)$. Note that, given the lower bound of Lemma~\ref{lem:1-1matching}, we would be able to directly derive the lower bound of Lemma~\ref{lem:keylemma} if the set $E$ of veto map edges contained a matching of size at least $\frac{1-\delta}{2}n$. Instead of finding such a matching, we instead
partition the set of voters $\V$ into the set $\vin$, which contains voters whose distance from $\o$ is strictly less than $d(\o,\p)/2$, and the set $\vout$, whose distance from $\o$ is at least $d(\o,\p)/2$. We then prove that the sub-graph of the veto map induced by vertices in $\vin$ contains in its edges a fractional matching of total size $\frac{1-\delta}{2}n-|\vout |$. Since each voter from $\vout$ contributes at least $d(\o,\p)/2$ to the optimal social cost and each edge of the fractional matching (whose vertices are both in $\vin$) also contributes (by Lemma \ref{lem:1-1matching}) at least $d(\o,\p)/2$ to the optimal social cost, the combined contribution from $\vin$ and $\vout$ is at least $\left(\frac{1-\delta}{2}n-|\vout| +|\vout |\right)d(\o,\p)/2=\left(\frac{1-\delta}{2}n\right)d(\o,\p)/2$, which implies the desired lower bound on $\SC(\o)$.
\begin{lemma}\label{lem:keylemma} 
For any $\delta \in [0,1)$, 
assume that $\p$ is the candidate output by a given execution of $\SimVeto$,
{\sl i.e.}, the algorithm returns the prediction.
Then we have 
$$\SC(\o) \geq \left(\frac{1-\delta}{2}n\right)\frac{d(\o,p)}{2}.$$
\end{lemma}
\begin{proof}
Let $\vin$ be the set of voters $v$ such that $d(v,\o) < \frac{d(\o,p)}{2}$ and let $\vout$ be the set of remaining voters, {\sl i.e.}, those with $d(v,\o) \geq \frac{d(\o,p)}{2}$. First, note that if $|\vout| \geq \frac{1-\delta}{2}n$ then the lemma is trivially true since $\SC(\o) \geq \sum_{v \in \vout} d(v,\o) \geq \left(\frac{1-\delta}{2}n\right) \frac{d(\o,p)}{2}$. Therefore, we henceforth focus on the case where $|\vout| < \frac{1-\delta}{2}n$ and let $x>0$ be such that $|\vout| = \frac{1-\delta}{2}n - xn$. Then, the contribution of voters in $\vout$ is
\begin{equation}\label{eq:Vout_contribution}
\sum_{v\in \vout} d(v,\o) \geq \left(\frac{1-\delta}{2}n - xn\right) \frac{d(\o,\p)}{2},
\end{equation}
and $|\vin| = n - |\vout| = \frac{1+\delta}{2}n + xn$. Our goal now is to show that the contribution of $\vin$ to $\SC(\o)$ compensates for the lack of enough voters in $\vout$. In particular, we will show that
%\[

\begin{align}
\label{eq:V_IN_contribution}
\sum_{v \in \vin}\d(v,\o) \geq xn \frac{d(\o,p)}{2},
\end{align}
%\]
and note that this would immediately imply the lemma.

Let $G = (V, E)$ be the veto map associated with the given execution of $\SimVeto$.
We now prove some useful inequalities regarding the veto map edge weights:
\begin{claim}\label{weight_constr1}
$\sum_{v\in \vin}w(v,v') \leq 1$ for all $v' \in \vin$. 
\end{claim}
\begin{proof}
Claim~\ref{weight_constr1} holds since every voter has 1 up-vote.  Formally,
for every voter $v'\in \vin$ we have
\[\sum_{v\in \vin}w(v,v')=\sum_{v\in \vin}\frac{f(v,\topc(v'))\cdot\frac{1+\delta}{1-\delta}}{\plu(\topc(v'))}\leq \sum_{v\in \V}\frac{f(v,\topc(v'))}{\plu(\topc(v'))}\cdot\frac{1+\delta}{1-\delta}=1,\]
where the last equation uses \eqref{Eq:total_downvote1}. Note that the reason \eqref{Eq:total_downvote1} applies and not \eqref{Eq:total_downvote2} is because $v'$ is in $\vin$ and hence $\topc(v')$ cannot be $\p$
($v'$ strictly prefers $\o$ over $\p$ since $\d(\o,v') < \d(\o,\p)/2 \leq (\d(\o,v')+\d(v',\p))/2$ using the definition of $\vin$ and the triangle inequality).
\end{proof}

\begin{claim}\label{weight_constr2}
$\sum_{v' \in \vin} w(v,v') \leq \frac{1+\delta}{1-\delta} \text{ for all $v \in \V$}.$ 
\end{claim}
\begin{proof}
Claim~\ref{weight_constr2} holds since every voter down-votes a total score of $\boosttotal$  throughout the execution of the algorithm.  Formally, 
\begin{align*}
    \sum_{v'\in \vin}w(v,v')&=\sum_{v'\in \vin}\frac{f(v,\topc(v'))\cdot\frac{1+\delta}{1-\delta}}{\plu(\topc(v'))}
    ~=~ \boosttotal \cdot \sum_{c \in \C} \sum_{v' \in \vin: \topc(v')=c} \frac{f(v,c)}{\plu(c)}\\
    & \leq \boosttotal \cdot \sum_{c \in \C} \sum_{v' \in \V: \topc(v')=c} \frac{f(v,c)}{\plu(c)}
     ~=~ \boosttotal \cdot \sum_{c \in \C} \plu(c) \cdot \frac{f(v,c)}{\plu(c)}\\
    & = \boosttotal \cdot \sum_{c \in \C} f(v,c)
     ~=~ \boosttotal, 
\end{align*}
where the last equality is by \eqref{Eq:total_time}.
\end{proof}

Our next claim, (Claim~\ref{weight_constr3}) provides a lower bound on the ``amount'' of up-votes from voters $v'\in \vin$ that are down-voted by some other voters $v\in \vin$. The way we obtain this bound is by showing that even if all the voters in $\vout$ spend all the time down-voting the up-votes of voters in $\vin$, there are still some up-votes left, which must have been down-voted by voters in $\vin$.

\begin{claim}\label{weight_constr3}
Let
$\ein\vcentcolon=\{(v,v')\in E:~v,v'\in \vin\}$ 
be
the subset of edges in the veto map for which both vertices are in $\vin$.
Then
we have 
$$\sum_{(v,v') \in \ein} w(v,v') \geq \frac{2xn}{1-\delta}.$$
\end{claim}
\begin{proof}
We first note that for every candidate $v'\in \vin$ we have $\sum_{v\in\V} f(v,\topc(v')) = \frac{1-\delta}{1+\delta}\cdot \plu(\topc(v'))$. This is implied by the fact that $\sum_{v\in\V} f(v,c) = \frac{1-\delta}{1+\delta}\cdot \plu(c)$ holds for every candidate $c\neq\p$ (by Equation~\eqref{Eq:total_downvote1}) and the fact that $\topc(v')$ cannot be $\p$ for any $v'\in\vin$ (because $d(v',\p)> d(\o,\p)/2 > d(v',\o)$ for all $v'\in \vin$, so $p$ cannot be the top candidate of $v'$). Therefore, we get
\begin{align}\label{eq:ui}
    \sum_{v' \in \vin} \sum_{v \in \V} w(v,v') = \sum_{v' \in \vin} \sum_{v \in \V} \frac{f(v,\topc(v'))\cdot \boosttotal }{\plu(\topc(v'))}=\sum_{v' \in \vin} \frac{ \plu(\topc(v'))}{\plu(\topc(v'))} = |\vin|.
\end{align}
Also, by Claim~\ref{weight_constr2} we get
\begin{align}\label{eq:uio}
    \sum_{v' \in \vin} \sum_{v \in \vout} w(v,v') = \sum_{v \in \vout} \sum_{v' \in \vin}w(v,v') \leq \sum_{v \in \vout} \boosttotal = \boosttotal \cdot |\vout|.
\end{align}
Therefore, we have
\begin{align*}
    \sum_{(v,v') \in \ein}  w(v,v') & = \sum_{v' \in \vin}\sum_{v \in \vin} w(v,v')\\
    & = \sum_{v' \in \vin} \sum_{v \in \V} w(v,v') - \sum_{v' \in \vin} \sum_{v \in \vout} w(v,v') \tag{since $\vin = \V \backslash \vout$}\\
    & \geq |\vin|- \boosttotal \cdot |\vout| \tag{using \eqref{eq:ui} and \eqref{eq:uio}}\\
    &= \left(\frac{1+\delta}{2}n +xn\right)-\boosttotal \cdot \left(\frac{1-\delta}{2}n - xn\right) \\
    &= \frac{2xn}{1-\delta}.\qedhere
\end{align*}
\end{proof}

We now use Lemma~\ref{lem:1-1matching} and Claims~\ref{weight_constr1}, \ref{weight_constr2} and \ref{weight_constr3} to lower bound the contribution of voters in $\vin$ toward the optimal social cost, {\sl i.e.}, $\sum_{v \in \vin}d(v, \o)$. 
Note that if we could find a matching $M \subseteq \ein$ of size $|M| \geq xn$, then using Lemma~\ref{lem:1-1matching} we would be done, {\sl i.e.}, \eqref{eq:V_IN_contribution} would be satisfied. We identify a fractional matching in $\ein$ whose size is at least $xn$. Specifically, for each edge $(v,v')\in \ein$ our fractional matching includes a fraction of this edge equal to
$$m(v,v') \vcentcolon= w(v,v') \cdot \frac{1-\delta}{2}.$$ 
To verify that this is a valid fractional matching, we first show that for any vertex $v\in \vin$ the total fraction of the edges adjacent to it (both incoming and outgoing) that are included in the matching is at most $1$.
Using Claim \ref{weight_constr1} and \ref{weight_constr2} we have:
\begin{equation}\label{eq:sumofweight}
    \sum_{v' \in \vin}m(v',v) + \sum_{v' \in \vin}m(v,v') = \frac{1-\delta}{2} \cdot \left(\sum_{v' \in \vin}w(v',v) + \sum_{v' \in \vin}w(v,v')\right) \leq \frac{1-\delta}{2} \cdot \left(1 + \frac{1+\delta}{1-\delta}\right) = 1. 
\end{equation}
Regarding the size of this matching, we get
\begin{equation}\label{eq:matching_size}
\sum_{(v,v')\in\ein} m(v,v') = \sum_{(v,v')\in\ein} w(v,v') \cdot \frac{1-\delta}{2} \geq \frac{1-\delta}{2} \cdot \frac{2xn}{1-\delta}= xn,
\end{equation}
where the inequality is implied by Claim~\ref{weight_constr3}.

We now lower bound the total contribution of voters in $\vin$ to the optimal social cost as follows:
\begin{align*}
    \sum_{v \in \vin} d(v,\o) &\geq \sum_{v \in \vin} \left(\sum_{v' \in \vin}m(v',v) + \sum_{v' \in \vin}m(v,v') \right)\cdot d(v,\o)\tag{using \eqref{eq:sumofweight}}\\
    & \geq \sum_{(v,v') \in E} m(v,v')\cdot (d(v,\o)+d(v',\o)) \tag{rearranging the sum }\\
    &\geq \sum_{(v,v') \in E} m(v,v')\cdot \frac{d(\o,p)}{2} \tag{by Lemma~\ref{lem:1-1matching}}\\
    & \geq xn \cdot \frac{d(\o,p)}{2}.\tag{using \eqref{eq:matching_size}} 
\end{align*}
For completeness,
we now show how the above,
combined with the contribution of voters from $\vout$ to the optimal social cost (which in turn is lower bounded by \eqref{eq:Vout_contribution}), allows us to prove the desired lower bound on the optimal social cost:
\begin{align*}
\SC(\o) 
&= \sum_{v \in \vout}d(v,\o) + \sum_{v \in \vin}d(v,\o)\\ 
&\geq \left(\frac{1-\delta}{2}n - xn\right)\frac{d(\o,p)}{2} + xn \frac{d(\o,p)}{2}\\ 
&\geq \left(\frac{1-\delta}{2}n\right) \frac{d(\o,p)}{2}.\qedhere
\end{align*}
\end{proof}

We are now ready to prove the main proposition of this section.
\begin{proof}[Proof of Proposition~\ref{prop:robustness_main}]
The social cost of the returned candidate $p$ can be upper bounded as follows: 
 {\allowdisplaybreaks
 \begin{align*}
     \sum_{v \in \V} d(v,p) &\leq \sum_{v} \sum_{c} f(v,c) \cdot d(v,p) \tag{using \eqref{Eq:total_time}}\\
     &\leq \sum_{v} \sum_{c} f(v,c) \cdot d(v,c) \tag{by Corollary~\ref{lem:activecandidate}}\\
     & \leq \sum_v \sum_c f(v,c) \cdot \left(d(v,\o) + d(\o,c)\right) \tag{triangle inequality}\\
     &= \SC(\o) + \sum_c \sum_{v} f(v,c) \cdot d(\o,c)\\
     &= \SC(\o) + \sum_{c \neq p}\sum_v f(v,c) \cdot d(\o,c) + \sum_v f(v,p) \cdot d(\o,p)\\
     &=\SC(\o) + \frac{1-\delta}{1+\delta} \left(\sum_c\plu(c) d(\o,c) + \frac{2\delta n}{1-\delta}d(\o,p)\right)\tag{using \eqref{Eq:total_downvote1} and \eqref{Eq:total_downvote2}}\\
      &=\SC(\o) + \frac{1-\delta}{1+\delta} \left(\sum_c\sum_{v: \topc(v) = c} d(\o,c) + \frac{2\delta n}{1-\delta}d(\o,p)\right)\\
      & \leq \SC(\o) + \frac{1-\delta}{1+\delta}\left( \sum_c\sum_{v: \topc(v) = c} (d(\o,v)+d(v,c))+ \frac{2\delta n}{1-\delta}d(\o,p)\right) \tag{triangle inequality}\\
      &\leq \SC(\o) + \frac{1-\delta}{1+\delta} \left(\sum_c\sum_{v: \topc(v) = c} 2d(\o,v)+ \frac{2\delta n}{1-\delta}d(\o,p)\right) \tag{since $c =\topc(v) \pref_v \o$}\\
      &\leq \SC(\o) + \frac{2(1-\delta)}{1+\delta}\SC(\o) + \frac{2\delta n}{1+\delta}d(\o,p)\\
       &\leq \frac{3-\delta}{1+\delta}\SC(\o) + \frac{2\delta n}{1+\delta}d(\o,p)\\
       & \leq \frac{3-\delta}{1+\delta}\SC(\o) + \frac{2\delta n}{1+\delta} \cdot \frac{2\SC(\o)}{\frac{1-\delta}{2}n} \tag{by Lemma~\ref{lem:keylemma}}\\
       & \leq \left(\frac{3-\delta}{1+\delta} + \frac{8\delta}{(1+\delta)(1-\delta)}\right)\SC(\o)\\
       & \leq \frac{3+4\delta+\delta^2}{(1+\delta)(1-\delta)} \SC(\o)
    ~\leq~ \frac{3+\delta}{1-\delta}\SC(\o).\qedhere
 \end{align*}}
 \end{proof}

\subsection{Robustness Bound when the Returned Candidate is not the Prediction}
\label{sec:robustness_not_prediction}

The following proposition shows
that the robustness bound is maintained even when $\SimVeto$ does not output the prediction.
\begin{proposition}
\label{prop:robustness_non_prediction_returned}
    For any $\delta \in [0,1)$, 
    assume that $a \in \C \setminus \{\p\}$ is the candidate output by a given execution of $\SimVeto$,
    {\sl i.e.}, the algorithm does not return the prediction.
    Then we have 
    $$\SC(a) \leq \frac{3+\delta}{1-\delta} \cdot \SC(\o).$$
\end{proposition}

First, we note that the approach taken in Section \ref{sec:robustness_prediction} will not work here.  In particular, the key Lemma~\ref{lem:keylemma} does not hold in general as the prediction can be arbitrarily far away from the optimal candidate.\footnote{For example, consider an instance with one voter, a candidate that is in the same location as the voter, and a second candidate (who is also the prediction) at distance 1 from the other two.  This instance violates Lemma \ref{lem:keylemma}.}
Instead, we show that if candidate $a\neq \p$ is returned, then she would have still been returned in an instance that is identical, except $a$ is the predicted candidate. 
In other words,
we prove Proposition \ref{prop:robustness_non_prediction_returned} by reducing instances in which the prediction is not the output to instances where it is while maintaining the distortion:

\begin{proposition}
\label{prop:reduction}
    For any $\delta \in [0,1)$, 
    assume that $a \in \C \setminus \{\p\}$ is the candidate output by a given execution of $\SimVeto$.
    Then 
    $\SimVeto$ also outputs $a$ when executed on the same preference profile, with candidate $a$ as the prediction.
\end{proposition}

Before presenting the proof of Proposition \ref{prop:reduction}, we first show how it implies Proposition \ref{prop:robustness_non_prediction_returned}.
\begin{proof}[Proof of Proposition \ref{prop:robustness_non_prediction_returned}]
    By Proposition \ref{prop:reduction},
    $a$ is returned by $\SimVeto$ when executed on the same preference profile as in the given execution, with candidate $a$ also being the prediction.
    That is, the new execution returns the new prediction (candidate $a$).
    The
    claim follows by Proposition \ref{prop:robustness_main}.
\end{proof}

We now present the proof of Proposition \ref{prop:reduction}.

\begin{proof}[Proof of Proposition \ref{prop:reduction}]
    We shall be comparing the two considered executions of $\SimVeto$, {\sl i.e.}, the one where $\p$ was the prediction (and $a$ was the output) 
    and the one where $a$ was the prediction.  To that end we shall refer to them as the ``$\p$ execution'' and the ``$a$ execution'', respectively.
    We need to show that $a$ is also the output in the $a$ execution.
    
    We first introduce some useful notation.  For any candidate $c \in \C$, any time point $t \in [0,1]$ and any $b\in \{a,\p\}$ we define
    \begin{itemize}
        \item $\dec_b(c,t)$ --- the amount of score decremented from $c$ up to time $t$, in the continuous interpretation of the $b$ execution.
        \item $\score_b(c,t)$ --- the score of $c$ at time $t$ in the continuous interpretation of the $b$ execution.
    \end{itemize}
    For both $b \in \{a,\p\}$ and for any fixed $c \in \C$, the function $\dec_b(c,\cdot)$ is piece-wise linear (in $t$) and can be computed using the round boundary time points $t_i$ from the discrete implementation of $\SimVeto$ (see Algorithm \ref{alg:simultaneous_veto}).
    Specifically, we have $\dec_b(c,0) = 0$, and if there were $k$ iterations in the While loop ({\sl i.e.}, $k$ rounds), then for each $i=1,\ldots,k$ and for any $t \in \left[t_{i-1},t_i\right]$
    (recall that $t_0 = 0$ and $t_k = 1$)
    we have
    \[
    \dec_b(c,t) = \dec_b(c,t_{i-1}) + n_c^i \cdot \boosttotal \cdot (t - t_{i-1}),
    \]
    where
    $n_c^i$ is the number of voters who down-voted $c$ in round $i$ (recall also that $\boosttotal$ is the down-voting rate per voter).
    The function $\score_b(c,\cdot)$ is defined as $\score_b(c,t) = s^b_c - \dec_b(c,t)$, where $s^b_c$ is the initial score of $c$ in the $b$ execution.  To summarize, we have
    
    \begin{observation}
    \label{obs:score+dec = init_score}
        \begin{itemize}
            \item   The functions $\dec_b(c,\cdot)$ and $\score_b(c,\cdot)$ are piece-wise linear and in particular continuous in $t$, for any fixed $c \in \C$ and $b\in\{a,\p\}$.
            \item   For any $c\in \C$, $t \in [0,1]$, and $b \in \{a,\p\}$, the initial score of $c$ in the $b$ execution, denoted $s^b_c$, satisfies $s^b_c = \dec_b(c,t) + \score_b(c,t)$.
        \end{itemize}
    \end{observation}

    We further observe that both executions are equivalent up to the time point where the score of $\p$ reaches 0 in the $a$ execution.  That is, we have:
    \begin{observation}
    \label{obs:equiv_before_p_dies}
    For any $c \in \C$ and for any $t$ such that $\score_a(\p,t) > 0$ we have $\dec_{\p}(c,t) = \dec_a(c,t)$.
    \end{observation}
    To see this, consider the implementation of $\SimVeto$ as given by Algorithm \ref{alg:simultaneous_veto}.
    Note that the only difference in the initialization phase of the two executions is the initial scores of $\p$ and $a$, 
    where in the $\p$ execution $\p$ gets the boost and in the $a$ execution $a$ gets the boost.
    But $a$ was output in the $\p$ execution, {\sl i.e.}, $a$ has positive score throughout the $\p$ execution and as such always belongs to the set of active candidates $A$. 
    Therefore, before $\p$'s score reaches 0 in the $a$ execution, every step of the While loop in Algorithm \ref{alg:simultaneous_veto} will be computed the same way in both executions.

    The following lemma captures the intuition that when $\p$ does not get the boost, the rest of the candidates can only be down-voted faster.
    \begin{lemma}
    \label{lem:dec_p<=dec_a}
        For any $c \in \C \setminus \{\p\}$, and for any $t \in [0,1]$, we have $\dec_{\p}(c,t) \leq \dec_a(c,t)$.
    \end{lemma}

    \begin{proof}
        Suppose towards contradiction that the lemma does not hold, {\sl i.e.},
        there is some candidate $c\neq \p$ and some time point $t$ for which $\dec_a(c,t) < \dec_{\p}(c,t)$.  
        Let $T$ be the set of such time points, {\sl i.e.},
        \[
        T := \{t \in [0,1] \mid \exists c \in \C \setminus \{\p\} \text{ such that } \dec_a(c,t) < \dec_{\p}(c,t)\}
        \]
        We note that for each $t \in T$ we have $t > 0$, because the amount of score decremented from any candidate at time $t=0$ equals 0 at both executions of the algorithm.
        
        Let $t_{\inf} = \inf(T)$. We note that $t_{\inf} \notin T$.  To see this, observe that for any $t \in T$ and candidate $c$ for which $\dec_a(c,t) < \dec_{\p}(c,t)$, there is some small enough $\epsilon > 0$ such that $\dec_a(c,t-\epsilon) < \dec_{\p}(c,t-\epsilon)$, that is $t-\epsilon \in S$.  This is clearly implied by the continuity of the functions $\dec_a(c,\cdot)$ and $\dec_{\p}(c,\cdot)$.
        
        Furthermore, note that $t_{\inf} < 1$, as otherwise $T$ is empty --- contradiction.
        Finally, the continuity of the functions $\dec_a(c,\cdot)$ and $\dec_{\p}(c,\cdot)$ also implies that at time $t = t_{\inf}$ there must exist a candidate $c \neq \p$ for which the following two assertions must hold:
        \begin{enumerate}
            \item $\dec_a(c,t_{\inf}) = \dec_{\p}(c,t_{\inf})$.
            \item There exists a small enough $\epsilon_0 > 0$ such that for any $0<\epsilon< \epsilon_0$ we have $\dec_a(c,t_{\inf} + \epsilon) < \dec_{\p}(c,t_{\inf} + \epsilon)$.
        \end{enumerate}
        In other words, the amount of score decremented from $c$ up until time $t_{\inf}$ was the same in both executions, but ever so slightly beyond time $t_{\inf}$, $\score(c)$ is decremented more in the $\p$ execution.
        In particular this implies  that at time $t_{\inf}$, the score of $c$ in the $\p$ execution was positive, {\sl i.e.}, $\score_{\p}(c,t_{\inf}) > 0$.  From here we also get:
        \begin{align*}
            \score_a(c,t_{\inf})    \geq \plu(c) - \dec_a(c,t_{\inf})
                                    =   \plu(c) - \dec_{\p}(c,t_{\inf})
                                    =   \score_{\p}(c,t_{\inf})
                                    > 0,
        \end{align*}
        where the first inequality holds by Observation \ref{obs:score+dec = init_score} since the initial score of each candidate is lower bounded by her plurality score, the first equality holds by bullet 1, the second equality holds since $c \neq \p$ and since the initial score of each candidate other than $\p$ equals her plurality score in the $\p$ execution, and the final inequality was discussed right before the above chain.

        To summarize, $c$'s score at $t_{\inf}$ was positive in both executions, but the decrement rate was higher in the $\p$ execution.
        But for this to hold, it must be the case that at time $t_{\inf}$ the number of voters who are 
        down-voting $c$ is larger in the $\p$ execution relative to the $a$ execution.
        In particular, there exists a voter $v$ who at time $t_{\inf}$ down-votes $c$ in the $\p$ execution, but in the $a$ execution she down-votes some other candidate $c' \neq c$, even though $c$ was also active in the $a$ execution at that time.  This implies that $v$ ranks $c'$ lower than $c$ and:
        
        \begin{itemize}
            \item $\score_a(c',t_{\inf}) > 0$ --- since $v$ down-votes $c'$ in the $a$ execution at time $t_{\inf}$ (only candidates with positive score are being down-voted at any given time).
            \item $\score_{\p}(c',t_{\inf}) = 0$ --- since otherwise $v$ would have down-voted $c'$ in the $\p$ execution at time $t_{\inf}$ (or some other active candidate that $v$ ranks lower than $c$).
        \end{itemize}
        Note that $c' \neq a$ since $a$ was output in the $\p$ execution (and in particular $\score_{\p}(a,t_{\inf}) > 0$).
        We also claim that $c' \neq \p$, since for any $t$ (and in particular for $t = t_{\inf}$) we have 
        \begin{align}
            \score_{\p}(\p,t) \geq \score_a(\p,t). \label{eq:score_p(p)_geq_score_a(p)}
        \end{align}
        To see this, note first that it is trivial for any $t$ for which $\score_a(\p,t) = 0$. For times $t$ in which $\score_a(\p,t) > 0$ we have
        \begin{align*}
            \score_{\p}(\p,t) = \plu(\p) + \boost - \dec_{\p}(\p,t)
                            = \plu(\p) + \boost - \dec_a(\p,t) 
                            = \score_a(\p,t) + \boost
                            \geq \score_a(\p,t),     
        \end{align*}
        where the first equality holds by Observation \ref{obs:score+dec = init_score}, the second holds by Observation \ref{obs:equiv_before_p_dies} and the third holds again by Observation \ref{obs:score+dec = init_score}.

        We have established that $c' \notin \{a,\p\}$, implying that the initial score of $c'$ in both executions is $\plu(c')$.  By Observation \ref{obs:score+dec = init_score}, this in turn implies:
        \begin{align*}
            \dec_a(c',t_{\inf}) = \plu(c') - \score_a(c',t_{\inf}) < \plu(c') - \score_{\p}(c',t_{\inf}) = \dec_{\p}(c',t_{\inf}),
        \end{align*}
        where the inequality holds by the two bullets above.
        In particular, this implies by definition that $t_{\inf} \in T$, a contradiction.        
    \end{proof}

Lemma \ref{lem:dec_p<=dec_a} shows that when $\p$ does not get the boost, the rest of the candidates can only be down-voted faster.  The following lemma upper bounds the extent to which that can happen.
\begin{lemma}
\label{lem:dec_a<=dec_p+boost}
    For any $c \in \C \setminus \{\p\}$, and for any $t \in [0,1]$, we have $\dec_a(c,t) \leq \dec_{\p}(c,t) + \boost$.
\end{lemma}

\begin{proof}
    Let $t \in [0,1]$. 
    %Let $c,t$ as in the lemma statement.
    We start with the following observation:
    \begin{observation}
    \label{obs:dec_p(p,t)_leq_dec_a(p,t)+boost}
        $\dec_{\p}(\p,t) \leq \dec_a(\p,t) + \boost$.
    \end{observation} 
    This holds since
    \begin{align*}
        \dec_{\p}(\p,t) = \plu(\p) + \boost - \score_{\p}(\p,t) \leq \plu(\p) + \boost - \score_a(\p,t) = \dec_a(\p,t) + \boost,
    \end{align*}
    where both equalities hold by Observation \ref{obs:score+dec = init_score} and the inequality holds by Inequality (\ref{eq:score_p(p)_geq_score_a(p)}).
    From here we get:
    \begin{align*}
        \sum_{c \in \C} \dec_a(c,t)   &=      \sum_{c \in \C} \dec_{\p}(c,t) \\
                                        &=      \left(\sum_{c \in \C \setminus \{\p\}}\dec_{\p}(c,t)\right) + \dec_{\p}(\p,t) \\
                                        &\leq   \left(\sum_{c \in \C \setminus \{\p\}}\dec_{\p}(c,t)\right) + \dec_a(\p,t) + \boost,
    \end{align*}
    where the first equality holds since the total amount of score decremented from all candidates up to time $t$ equals $t\cdot n\cdot \boosttotal$ regardless of the prediction's identity, and the inequality holds by Observation \ref{obs:dec_p(p,t)_leq_dec_a(p,t)+boost}.  By cancelling out the $\p$ term from both sides, we get 
    \[
    \sum_{c \in \C \setminus \{\p\}} \dec_a(c,t) \leq \left(\sum_{c \in \C \setminus \{\p\}}\dec_{\p}(c,t)\right) + \boost,
    \]
    which in turn implies
    \[
    \sum_{c \in \C \setminus \{\p\}} \left(\dec_a(c,t)- \dec_{\p}(c,t)\right) \leq \boost.
    \]
    By Lemma \ref{lem:dec_p<=dec_a}, all terms in this sum are non-negative, implying in particular that each of the terms is also upper-bounded by $\boost$.  The claim follows.
\end{proof}

To conclude the proof of Proposition \ref{prop:reduction}, we show that for any $0\leq t < 1$ we have $\score_a(a,t) > 0$.  This would imply that $a$ belongs to the set $A$ at the end of Algorithm \ref{alg:simultaneous_veto}, and therefore $a$ would be the output in the $a$ execution, as desired.
To that end, we have
\begin{align*}
    \score_a(a,t) = \plu(a) + \boost - \dec_a(a,t) \geq \plu(a) - \dec_{\p}(a,t) = \score_{\p}(a,t) > 0,
\end{align*}
where the first equality holds by Observation \ref{obs:score+dec = init_score},
the first inequality holds by Lemma \ref{lem:dec_a<=dec_p+boost},
the second equality holds again by Observation \ref{obs:score+dec = init_score},
and the second inequality holds by our assumption that $a$ was output in the $\p$ execution.    
\end{proof}


